Online vs. Offline Adaptive Domain Randomization Benchmark

Physics simulators have shown great promise for conveniently learning reinforcement learning policies in safe, unconstrained environments. However, transferring the acquired knowledge to the real world can be challenging due to the reality gap. To this end, several methods have been recently proposed to automatically tune simulator parameters with posterior distributions given real data, for use with domain randomization at training time. These approaches have been shown to work for various robotic tasks under different settings and assumptions. Nevertheless, existing literature lacks a thorough comparison of existing adaptive domain randomization methods with respect to transfer performance and real-data efficiency. In this work, we present an open benchmark for both offline and online methods (SimOpt, BayRn, DROID, DROPO), to shed light on which are most suitable for each setting and task at hand. We found that online methods are limited by the quality of the currently learned policy for the next iteration, while offline methods may sometimes fail when replaying trajectories in simulation with open-loop commands. The code used will be released at https://github.com/gabrieletiboni/adr-benchmark.

==> sections/03b_problem_formulation_v2.tex <==
% 1. The real world MDP
Consider the real environment to be modeled by a discrete-time dynamical system, with a continuous state space $\mathcal{S} \in \mathbb{R}^{n_s}$, continuous action space $\mathcal{A} \in \mathbb{R}^{n_a}$, and initial state distribution $\mu(s_0)$.
The system dynamics are therefore described by the transition probability density function $\mathcal P(s_{t+1} | s_{t}, a_{t})$, where the state at $t+1$ depends on the state $s_{t}$ and the action $a_{t}$ taken at time step $t$.
At each step, the agent is given a scalar reward feedback $r_t$ according to the function $R(s_t, a_t)$, assumed to be deterministic for the sake of notation simplicity.
Overall, this environment forms a Markov Decision Process (MDP) described by the tuple $\mathcal M = \left<\mathcal S, \mathcal A, \mathcal P, \mu, R\right>$.

% 2. Real-world RL
The goal of an RL agent is then to find an optimal stochastic policy $\pi(a_t | s_t)$ in order to maximize the expected return, as

\begin{equation}
    \pi^{*} =\underset{\pi }{\argmax } \ E_{\pi , \mathcal{P}, \mu _{0}}\left[ \ \sum _{t=0}^{T} \gamma ^{t} r_{t}\right]
\end{equation}

with discount factor $\gamma \in (0,1]$.
% 3. However, ...
However, optimizing $\pi^*$ directly in the target environment is not feasible, as sampling rollouts from $\mathcal{M}$ is assumed to be expensive; instead, the policy is optimized in a proxy \textit{source} MDP, corresponding to the simulated environment.

% 4. Simulated MDP formulation
The simulated environment follows a similar structure, but is further parameterized by the dynamics parameters $\xi \in \mathbb R^{n_\xi}$, e.g. masses, friction coefficients, robot link sizes.
The dynamics of the simulated system are therefore additionally conditioned on the system dynamics $\xi$: $\mathcal P_\xi(s_{t+1} | s_{t}, a_{t}, \xi)$.
Thus, the simulated environment forms an MDP described by the tuple $\mathcal M_{\xi} = \left<\mathcal S, \mathcal A, \mathcal P_\xi, \mu, R\right>$.
For the purpose of sim-to-real transfer, we assume that both MDPs share their state and action spaces $\mathcal{S}$ and $\mathcal{A}$, the initial state distribution $\mu$ and the reward function $R$, but vary in state transition dynamics.

In this work, we assume $\xi$ to be random variables that obey a parametric distribution $\xi \sim p_{\phi}(\xi)$---referred to as the source domain distribution---parametrized by $\phi$.
% 5. Simulated RL
Therefore, in the domain randomization setting, the goal is to train a robust policy in simulation over the source domain distribution, resulting in the additional outer expectation term:
\begin{equation}
    \pi_{\phi}^{*} =\underset{\pi }{\argmax } \ \mathbb{E}_{\xi \sim p_{\phi } (\xi )}\left[ E_{\pi, \mathcal{P}_{\xi } ,\mu _{0}}\left[ \ \sum _{t=0}^{T} \gamma ^{t} r_{t}\right]\right].
\end{equation}

% 6. ADR
Given these preliminaries, the goal of the Adaptive Domain Randomization (ADR) methods taken into account in this work is to find a parameterization $\phi^*$ for which the return in the target domain $\mathcal{M}$ is maximized when acting with the optimal policy $\pi_{\phi}^{*}$:
\begin{equation} \label{eq:nu_star}
    \phi ^{*} =\underset{\phi }{\argmax } \ E_{\pi _{\phi }^{*} , \mathcal{P}, \mu _{0}}\left[ \ \sum _{t=0}^{T} \gamma ^{t} r_{t}\right].
\end{equation}

Different ADR methods vary in terms of the assumption behind what data is available to perform the optimization in (\ref{eq:nu_star}): some assume that policies can be arbitrarily rolled out from $\mathcal{M}$ (\textit{online ADR;}~\cite{simopt2019,bayrn2021}), others assume only a pre-collected dataset $\mathcal{D} = \{(s_0, a_0, s_1, r_1), \dots , (s_{T-1}, a_{T-1}, s_T, r_T) \}$ to be available (\textit{offline ADR;}~\cite{dropo2022,droid2021}), while others assume no real-world data to be available at all (\textit{Unsupervised ADR};~\cite{ADRrubikscube,ADR}).
